Labelling unlabelled videos from scratch with multi-modal self-supervision

A large part of the current success of deep learning lies in the effectiveness of data -- more precisely: labelled data. Yet, labelling a dataset with human annotation continues to carry high costs, especially for videos. While in the image domain, recent methods have allowed to generate meaningful (pseudo-) labels for unlabelled datasets without supervision, this development is missing for the video domain where learning feature representations is the current focus. In this work, we a) show that unsupervised labelling of a video dataset does not come for free from strong feature encoders and b) propose a novel clustering method that allows pseudo-labelling of a video dataset without any human annotations, by leveraging the natural correspondence between the audio and visual modalities. An extensive analysis shows that the resulting clusters have high semantic overlap to ground truth human labels. We further introduce the first benchmarking results on unsupervised labelling of common video datasets Kinetics, Kinetics-Sound, VGG-Sound and AVE.

==> figs/clusters.tex <==

\begin{figure}[t!]
\captionsetup[subfigure]{labelformat=empty}
\captionsetup[subfigure]{oneside,margin={0.1cm,0cm}}
    \centering
    \begin{subfigure}[t]{0.09\textwidth}
        \centering
        \caption{\tiny \texttt{barn swallow calling}}
        \includegraphics[width=\textwidth]{figs/random-clusters-12.png}
    \end{subfigure}%
    \hfill
    \begin{subfigure}[t]{0.09\textwidth}
        \centering
        \caption{\tiny \texttt{splashing water}\newline }
        \includegraphics[width=\textwidth]{figs/random-clusters-14.png}
    \end{subfigure}%
    \hfill
    \begin{subfigure}[t]{0.09\textwidth}
        \centering
        \caption{\tiny \texttt{fire truck siren}\newline}
        \includegraphics[width=\textwidth]{figs/random-clusters-16.png}
    \end{subfigure}
    \hfill
    \begin{subfigure}[t]{0.09\textwidth}
        \caption{\tiny \texttt{playing trumpet}\newline}
        \includegraphics[width=\textwidth]{figs/random-clusters-2.png}
    \end{subfigure}
    \hfill
    \begin{subfigure}[t]{0.09\textwidth}
        \centering
        \caption{\tiny \texttt{eagle screaming}\newline}
        \includegraphics[width=\textwidth]{figs/random-clusters-3.png}
    \end{subfigure}
    \hfill
    \begin{subfigure}[t]{0.09\textwidth}
        \centering
        \caption{\tiny \texttt{car engine idling}\newline}
        \includegraphics[width=\textwidth]{figs/random-clusters-4.png}
    \end{subfigure}
    \hfill
    \begin{subfigure}[t]{0.09\textwidth}
        \centering
        \caption{\tiny \texttt{slot machine  }\newline}
        \centering
        \includegraphics[width=\textwidth]{figs/random-clusters-5.png}
    \end{subfigure}
    \hfill
    \begin{subfigure}[t]{0.09\textwidth}
        \centering
        \caption{\tiny \texttt{tapping guitar}\newline}
        \includegraphics[width=\textwidth]{figs/random-clusters-18.png}
    \end{subfigure}%
    \hfill
    \begin{subfigure}[t]{0.090\textwidth}
        \centering
        \caption{\tiny \texttt{playing bagpipes}\newline}
        \includegraphics[width=\textwidth]{figs/random-clusters-7.png}
    \end{subfigure}
    \begin{subfigure}[t]{0.090\textwidth}
        \centering
        \caption{\tiny \texttt{lions growling}\newline}
        \includegraphics[width=\textwidth]{figs/r10.png}
    \end{subfigure}
    \caption{\textbf{Ten randomly chosen clusters}, unsupervisedly obtained from the VGG-Sound dataset are shown, with six randomly chosen videos' snapshots.
    The ground-truth classes are indicated by the bounding box color and the cluster's greedily matched ground-truth class name is on top.
    \textit{Best viewed with sound} (in the supplementary material). 
    \label{fig:viz}}
\vspace{-10pt}
\end{figure}

==> tabs/appx_further_ablation.tex <==
\setlength{\tabcolsep}{4pt}
  \setlength{\fboxsep}{1.2pt}
  \centering
  \captionof{table}{ \textbf{Ablation}
  of multi-modality, audio-visual \ul{A}lignment and
  \ul{G}aussian  marginals. 
  \ul{D}ecorrelated \ul{H}eads.  Models are evaluated at 100 epochs on the VGG-Sound dataset.
  \label{tab:appx:blation-ours}}
  \vspace{1em}
  \begin{tabular}{l @{\hskip 5pt} ccccc @{\hskip 5pt} c }
  \toprule
     Method         &  \faFileImageO &  (\colorbox{blue!30}{\faVolumeUp} {\setlength{\fboxsep}{1.7pt}\colorbox{green!30}{\faVideoCamera}}) & A? & G.? & DH? & \textbf{NMI} \\ %
    \midrule                                                         %
     SeLa          & \cmark & \xmark & --      & --     & --     & 20.1         \\ 
     Concat        & \xmark & \cmark & --      & \xmark & \xmark & 24.7         \\
     Ours          & \xmark & \cmark & \xmark  & \xmark & \xmark & 51.9         \\ 
    \midrule
     Ours          & \xmark & \cmark & \xmark  & \cmark & \cmark & 52.6         \\
     Ours          & \xmark & \cmark & \cmark  & \xmark & \cmark & 52.7         \\
     Ours          & \xmark & \cmark & \cmark  & \cmark & \xmark & 52.4         \\
    \midrule
     Ours          & \xmark & \cmark & \cmark & \cmark  & \cmark & 53.2   \\
    \bottomrule
  \end{tabular}

